DeepScholar-Bench: A Live Benchmark and Automated Evaluation for Generative Research Synthesis

The ability to research and synthesize knowledge is central to human expertise and progress. A new class of AI systems--designed for generative research synthesis--aims to automate this process by retrieving information from the live web and producing long-form, cited reports. Yet, evaluating such systems remains an open challenge: existing question-answering benchmarks focus on short, factual answers, while expert-curated datasets risk staleness and data contamination. Neither captures the complexity and evolving nature of real research synthesis tasks. We introduce DeepScholar-bench, a live benchmark and automated evaluation framework for generative research synthesis. DeepScholar-bench draws queries and human-written exemplars from recent, high-quality ArXiv papers and evaluates a real synthesis task: generating a related work section by retrieving, synthesizing, and citing prior work. Our automated framework holistically measures performance across three key dimensions--knowledge synthesis, retrieval quality, and verifiability. To further future work, we also contribute DeepScholar-ref, a simple, open-source reference pipeline, which is implemented on the LOTUS framework and provides a strong baseline. Using DeepScholar-bench, we systematically evaluate prior open-source systems, search agents with strong models, OpenAI's DeepResearch, and DeepScholar-ref. We find DeepScholar-bench is far from saturated: no system surpasses a geometric mean of $31\%$ across all metrics. These results highlight both the difficulty and importance of DeepScholar-bench as a foundation for advancing AI systems capable of generative research synthesis. We make our benchmark code and data available at https://github.com/guestrin-lab/deepscholar-bench.

==> Sections/Discussion.tex <==

\subsection{Limitations}

% \subsection{Future Work}

==> Sections/agreement.tex <==
\begin{table}[t]
\centering
\caption{
Confusion matrices comparing human and LLM judgments on organization, Nugget importance judgments, and Reference-importance judgments, where in each table rows and columns represent human and LLM judgments}.

\small
\begin{subtable}[t]{0.35\linewidth}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lccc}
        \toprule
        \multicolumn{4}{c}{\textbf{Organization}} \\
        \midrule
        \textbf{Human / LLM} & Ref. Rep. & Gen. Rep. & Tie \\
        \midrule
        Reference Report   & 10.4\% & 15.6\% & 9.1\% \\
        Generated Report   & 2.6\%  & 37.7\% & 11.7\% \\
        Tie                & 1.3\%  & 3.9\%  & 7.8\% \\
        \bottomrule
    \end{tabular}
    \label{tab:org_confusion}
\end{subtable}
\hfill
\begin{subtable}[t]{0.29\linewidth}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lccc}
        \toprule
        \multicolumn{4}{c}{\textbf{Nugget Importance}} \\
        \midrule
        \textbf{Human / LLM} & Vital & Okay & Irrel. \\
        \midrule
        Vital      & 50.0\% & 12.1\% & 0.0\% \\
        Okay       & 12.1\% & 17.4\% & 0.0\% \\
        Irrelevant & 4.5\%  & 3.8\%  & 0.0\% \\
        \bottomrule
    \end{tabular}
    \label{tab:nugget_confusion}
\end{subtable}
\hfill
\begin{subtable}[t]{0.3\linewidth}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{lcc}
        \toprule
        \multicolumn{3}{c}{\textbf{Reference Essentiality}} \\
        \midrule
        \textbf{Human / LLM} & non-ess. & ess. \\
        \midrule
        non-essential & 40.2\% & 9.8\% \\
        essential     & 24.2\% & 25.7\% \\
        \bottomrule
    \end{tabular}
    \label{tab:ref_confusion}
\end{subtable}

\label{tab:human_llm_confusion}
\end{table}

==> algs/formatting.tex <==
\DontPrintSemicolon
% \small

\SetKwIF{If}{ElseIf}{Else}{if}{}{else if}{else}{endif}
\SetKwFor{For}{for}{}{}
\SetKwFor{ForEach}{for each}{}{}
\LinesNumbered


==> tables/verifiability_res.tex <==
\begin{table*}[!t]
    \centering
    \caption{Verifiability Evaluation. We report the citation precision (cite-p), citation-recall (cite-R) and citation F1 (cite-F1) across each baseline.}
    \begin{tabular}{ccc|c}
    \toprule
         & Cite-P  & Cite-R &  Cite-F1 \\
    \midrule
    \multicolumn{4}{c}{\emph{Open Source Research Synthesis Systems}}\\
     \midrule{}
         DeepResearcher & .006 & .025 & .037  \\
         STORM & .205 & .117 & .149  \\
         OpenScholar & .321 & .223 & .263  \\
         LOTUS Pipeline & .683 & .491 & .571  \\
     \midrule
     \multicolumn{4}{c}{\emph{Search AI's}}\\
     \midrule
     Llama-4-Scout & .075 & .042 & .054  \\
     gpt-4o-mini & .104 & .032 & .049  \\
     gpt-4o & .118 & .050 & .070  \\
     o1 & .087 & .040 & .054  \\
     \midrule
     \multicolumn{4}{c}{\emph{Commercial Systems}}\\
     \midrule
     OpenAI Deepresearch & .628 & .359 & .457 \\
    
     \midrule        
    \end{tabular}  
    \label{tab:res_verifiability}
\end{table*}



